I can listen but cannot read: An evaluation of two-tower multimodal systems for instrument recognition

Music two-tower multimodal systems integrate audio and text modalities into a joint audio-text space, enabling direct comparison between songs and their corresponding labels. These systems enable new approaches for classification and retrieval, leveraging both modalities. Despite the promising results they have shown for zero-shot classification and retrieval tasks, closer inspection of the embeddings is needed. This paper evaluates the inherent zero-shot properties of joint audio-text spaces for the case-study of instrument recognition. We present an evaluation and analysis of two-tower systems for zero-shot instrument recognition and a detailed analysis of the properties of the pre-joint and joint embeddings spaces. Our findings suggest that audio encoders alone demonstrate good quality, while challenges remain within the text encoder or joint space projection. Specifically, two-tower systems exhibit sensitivity towards specific words, favoring generic prompts over musically informed ones. Despite the large size of textual encoders, they do not yet leverage additional textual context or infer instruments accurately from their descriptions. Lastly, a novel approach for quantifying the semantic meaningfulness of the textual space leveraging an instrument ontology is proposed. This method reveals deficiencies in the systems' understanding of instruments and provides evidence of the need for fine-tuning text encoders on musical data.

==> ISMIR2024_template.tex <==
% % -----------------------------------------------
% % Template for ISMIR Papers
% % 2023 version trained based on previous ISMIR templates

% % Requirements :
% % * 6+n page length maximum
% % * 10MB maximum file size
% % * Copyright note must appear in the bottom left corner of first page
% % * Clearer statement about citing own work in anonymized submission
% % (see conference website for additional details)
% % -----------------------------------------------

% \documentclass{article}
% \usepackage[T1]{fontenc} % add special characters (e.g., umlaute)
% \usepackage[utf8]{inputenc} % set utf-8 as default input encoding
% \usepackage{ismir,amsmath,cite,url}
% \usepackage{graphicx}
% \usepackage{color}
% \DeclareMathOperator*{\argminB}{argmax}
% \usepackage{amssymb}
% \usepackage{subcaption}
% \usepackage{xcolor}
% \usepackage{soul}

% \usepackage{lineno}
% \linenumbers

% % Title. Please use IEEE-compliant title case when specifying the title here,
% % as it has implications for the copyright notice
% % ------
% % \title{Paper Template for ISMIR \conferenceyear}

% \title{I can listen but cannot read: \\ An evaluation of two-tower multimodal systems \\ for instrument recognition}

% % Note: Please do NOT use \thanks or a \footnote in any of the author markup

% % Single address
% % To use with only one author or several with the same address
% % ---------------
% %\oneauthor
% % {Names should be omitted for double-blind reviewing}
% % {Affiliations should be omitted for double-blind reviewing}

% % Two addresses
% % --------------
% %\twoauthors
% %  {First author} {School \\ Department}
% %  {Second author} {Company \\ Address}

% % Three addresses
% % --------------\input{ISMIR2021_paper.tex}

% \threeauthors
%   {First Author} {Affiliation1 \\ {\tt author1@ismir.edu}}
%   {Second Author} {\bf Retain these fake authors in\\\bf submission to preserve the formatting}
%   {Third Author} {Affiliation3 \\ {\tt author3@ismir.edu}}

% % Four or more addresses
% % OR alternative format for large number of co-authors
% % ------------
% %\multauthor
% %{First author$^1$ \hspace{1cm} Second author$^1$ \hspace{1cm} Third author$^2$} { \bfseries{Fourth author$^3$ \hspace{1cm} Fifth author$^2$ \hspace{1cm} Sixth author$^1$}\\
% %  $^1$ Department of Computer Science, University , Country\\
% %$^2$ International Laboratories, City, Country\\
% %$^3$  Company, Address\\
% %{\tt\small CorrespondenceAuthor@ismir.edu, PossibleOtherAuthor@ismir.edu}
% %}

% % For the author list in the Creative Common license, please enter author names. 
% % Please abbreviate the first names of authors and add 'and' between the second to last and last authors.
% \def\authorname{F. Author, S. Author, and T. Author}

% % Optional: To use hyperref, uncomment the following.
% %\usepackage[bookmarks=false,pdfauthor={\authorname},pdfsubject={\papersubject},hidelinks]{hyperref}
% % Mind the bookmarks=false option; bookmarks are incompatible with ismir.sty.

% \sloppy % please retain sloppy command for improved formatting

% \begin{document}

% %
% \maketitle
% %
% \begin{abstract}
% Music two-tower multimodal systems integrate audio and text modalities into a joint audio-text space, enabling direct comparison between songs and their corresponding words. These systems enable new approaches for classification and retrieval, leveraging both modalities. Despite the promising results they have shown for zero-shot classification and retrieval tasks, closer inspection of the embeddings is needed. This paper evaluates the inherent zero-shot properties of joint audio-text spaces for the case-study of instrument recognition. We present an evaluation and analysis of two-tower systems for zero-shot instrument recognition, and a detailed analysis of the properties of the pre-joint and joint embedding spaces. 

% Our findings suggest that audio encoders alone demonstrate good quality, while challenges remain within the text encoder or joint space projection. Specifically, two-tower systems exhibit sensitivity towards specific words, favoring generic prompts over musically informed ones. Despite the large size of textual encoders, they do not yet leverage additional textual context or infer instruments accurately from their descriptions. Lastly, a novel approach for quantifying the semantic meaningfulness of the textual space leveraging an instrument ontology is proposed. This method reveals deficiencies in the systems' understanding of instruments and provides evidence of the need for fine-tuning text encoders on musical data.

% \end{abstract}
% %

% \section{Introduction}\label{sec:introduction}
% Multiclass classification has been a heavily researched topic in Music Information Retrieval (MIR) with many concrete applications such as genre, instrument and emotion recognition~\cite{genre_classification_review_ndou_2021, music_emotion_recognition_survey_donghong_2022, music_classification_beyond_supervised_learning_won_2021, a_survey_music_classification_2011}. Despite the success of Deep (DL) systems for such tasks, recurring deficiencies persist among these problems. These are: (1) the limited availability of large-scale annotated datasets curated by experts, (2) the restricted capability of these systems to infer only a set of predefined classes.

% \begin{figure}
%  \centerline{\includegraphics[width=\columnwidth, height=3.5cm]{figs/final_two_tower_system_overview.jpg}}
%  \caption{Figure of a pipeline for two-tower multimodal systems. A separate model for each modality is used and their individual representations are projected to a joint audio-text space through a Multi Layer Perceptron. This enables direct comparison between audio and textual data.}
%  \label{fig:abstract_two_tower_system}
% \end{figure}

% % A solution to the first problem is to decouple the representation learning from classification and use the plethora of unannotated songs that are available with self-supervised and contrastive learning to obtain task-agnostic representations~\cite{mert_acoustic_music_understanding_self_yizhi_2023, towards_learning_universal_audio_rep_wang_2021, masked_spectrogram_modeling_daisuke_2022}. These representations can be used as input data to train a classifier for the set of classes that are of interest.

% Music is an ever-evolving art form and as a result, there is an inherent need to make these systems adaptable to new terms/classes~\cite{classification_as_culture_jennifer_2008, categorical_ambiguity_genre_Venrooij_2018, Hennequin2018AudioBD} and infer task-agnostic representations that can be useful for a plethora of downstream tasks with representation learning \cite{pann_kong_2019, hts_at_a_hierarchical_Ke_2022, towards_learning_universal_audio_rep_wang_2021}. Zero-shot learning (ZSL) is focused on estimating a classifier capable of inferring unseen, new classes without annotated examples~\cite{zero_shot_factored_linear_huang_2020, zero_shot_learning_for_audio_choi_2019, zeroshot_semantic_embeddings_huang_2020, zershot_class_label_embeddings_2019}. ZSL if often achieved in two ways: (1) by decomposing each class into attributes and inferring unseen classes through their related attributes (e.g. genres decomposed to presence or absence of instruments~\cite{zero_shot_learning_for_audio_choi_2019}) or (2) using word embeddings from Language Models (LM)~\cite{zero_shot_learning_for_audio_choi_2019, zeroshot_semantic_embeddings_huang_2020, zershot_class_label_embeddings_2019}. The success of contextualized Large Language Models (LLM) has driven the research community predominantly towards the second solution, as it doesn't require experts to define attributes and the mapping between classes and attributes~\cite{Pratt_2023_ICCV, Ge_2023_CVPR, Goyal_2023_CVPR}.

% As a result, ZSL for audio classification is primarily focused on connecting the audio and semantic representation spaces. This interconnection can happen in 2 main ways: (1) mapping the audio representations to text space~\cite{zeroshot_semantic_embeddings_huang_2020, zero_shot_learning_for_audio_choi_2019}, or (2) mapping both of the spaces to a new, joint audio-text space~\cite{zershot_class_label_embeddings_2019, muscall_manco_2022, mulan_a_joint_embedding_qinqing_2022, clap_learning_audio_concepts_elizalde_2023}. The systems of the second category are named two-tower multimodal systems, where pre-trained audio models and LMs are used as the audio and text encoders respectively. Representations obtained from each modality are then mapped to a joint audio-text space and systems are jointly optimized such that the audio and text representation are close in the joint space (e.g. the phrase ``A rock song track'' is similar to the recording of a ``rock'' song). We will call such representations as embeddings from here on.

% This work aims to better understand the properties of existing two-tower systems. We use instrument classification as a case-study to provide insights into the presence (or absence) of semantic properties in the audio, text or joint spaces in addition to reporting classification metrics. Concretely, we consider 3 systems: MusCALL~\cite{muscall_manco_2022}, a CLAP~\cite{clap_learning_audio_concepts_elizalde_2023, laion_clap_Wu_2023} model trained on speech and music datasets, and a CLAP model trained on music data~\cite{laion_clap_Wu_2023}. We evaluate the performance of these systems on instrument classification using the TinySOL dataset~\cite{TinySOL}. We would like to highlight that multimodal DL models typically excel at simple tasks and datasets like this.

% Furthermore, a novel approach for quantifying the semantic meaningfulness of textual encoders for instrument recognition is proposed.

% % In more detail, it is proposed to form (<anchor>, <positive>, <negative>) triplets with terms that are included in established instrument ontologies. <anchor> has to be more similar to <positive> than <negative> and based on that, we calculate the accuracy of text encoders as a proxy task to quantify the knowledge they posses about musical instruments. 

% For reproducability, our experiments are performed on open-source datasets and the code used to reproduce our experiments is made publicly available\footnote{\url{https://github.com/anonymous/submission}}.

% \section{Related work}\label{sec:related_work}

% \subsection{Zero-shot transfer}\label{subsec:zeroshot_learning}

% ZSL focusses on estimating classifiers for novel, unseen classes without annotated examples. Two-tower systems are not primarily optimized for ZSL but due to the pretrained textual encoder, novel words or phrases can be interpreted during inference. This property is known as zero-shot transfer (ZST)~\cite{lit_zero_shot_transfer_Zhai_2022}.

% Side-information can be used in multiple ways that fall in two categories: (1) decomposing classes into shared attributes and (2) using LMs to represent this information as a text embedding. Despite its success, the first solution requires experts to effectively estimate the relevance of attributes and several classes and is a costly activity. As a result and due to the remarkable results obtained trough contextualized LLMs, research has focused on the second option.

% Generally,  the methodology can be broken down into 3 components: (1) an audio encoder, (2) a textual encoder and (3) a projection to a common space. General purpose audio DL models have been used as the audio encoder ranging from VGGish~\cite{vggish_simonyan_2014}, PANN~\cite{pann_kong_2019}, HTS-AT~\cite{hts_at_a_hierarchical_Ke_2022} and Audio Spectrogram Transformers~\cite{audio_spectrogram_transformer_2021}. For the textual encoder, distributional LMs like GloVE~\cite{glove_pennington_2014}, Word2Vec~\cite{word2vec_mikolov_2013} and contextualized LMs like BERT~\cite{bert_devlin_2019} have been thoroughly tested. As each modality produces heterogenous representations, different methods of establishing comparability have been tested. This is predominantly achieved through projecting audio to text/semantic space or a novel \cite{zero_shot_factored_linear_huang_2020, zero_shot_learning_for_audio_choi_2019, zeroshot_semantic_embeddings_huang_2020}, joint audio-text space \cite{muscall_manco_2022, mulan_a_joint_embedding_qinqing_2022, clap_learning_audio_concepts_elizalde_2023}.


% \subsection{Two-tower multimodal systems}\label{subsec:two_tower_multimodal_systems}
% Multimodal systems aim to represent data with additional knowledge from multiple modalities. Examples are audio combined with images~\cite{zero_shot_audio_image_dogan_2022}, text~\cite{zero_shot_learning_for_audio_choi_2019, Du2023JointMA} or a combination of those.

% Two-tower multimodal systems focus on combining the textual and audio modalities through projecting them in a joint audio-text space. In that space, words that are relevant to a specific song will produce embeddings that will be close in terms of some similarity metric. An abstract figure of a two-tower system is presented in figure \ref{fig:abstract_two_tower_system}. Information flowing through the audio encoder or textual encoder is also referred to as the audio and textual branch respectively. We are also interested in the embeddings obtained through the encoders before projecting them to the joint audio-text space. We will call them as the pre-joint space from now on.

% The text used during training is usually a description of a song and will be referred to as a caption. The text used during inference will be referred to as a prompt. 

% MusCALL~\cite{muscall_manco_2022} combined a ResNET-50 for audio~\cite{resnet_50_2016} with a Transformer for text encoding~\cite{Vaswani2017AttentionIA}, optimized jointly over InfoNCE contrastive loss~\cite{oord2018representation}. Additionally, a weighing mechanism based on caption-caption similarity was incorporated between negative audio-caption pairs. This is based on the premise that similar captions will be given to similar audio. The audio used is private but the training code is publicly available and used for this work.

% MuLan~\cite{mulan_a_joint_embedding_qinqing_2022} experimented with ResNET-50 as well as Audio Spectrogram Transformers~\cite{audio_spectrogram_transformer_2021} for audio encoding and a pretrained BERT model for the text branch and jointly optimized over the Contrastive Multiview Coding loss~\cite{Tian2019ContrastiveMC}, which is a cross-modal extension of InfoNCE. Neither the data nor the code is available.

% \begin{figure}
%  \centerline{\includegraphics[width=\columnwidth]{figs/final_top2_difference.png}}
%  \caption{The histogram of top-2 class similarities for every song in TinySOL. The CLAP models tend to be not very confident while the metrics are greater than the overconfident MusCALL with the worst metrics.}
%  \label{fig:top_2_confidence_difference}
% \end{figure}

% LAION-CLAP tested 6 different combinations of audio and text embedding models, the best one of which was HTS-AT with RoBERTa~\cite{Liu2019RoBERTaAR}. The latter is the one that will be used in this paper. They formed the LAION-Audio-630k dataset by combining AudioCaps, CLotho and Audioset.

% Generally, research for two-tower systems is limited to testing different combinations of audio and text encoders, optimized jointly over a form of contrastive loss and modalitiy fusion without. We believe that closer inspection of their embeddings and evaluation protocol is needed.

% \section{Evaluation of two-tower systems}\label{sec:experiments_run}

% \subsection{Dataset and models}\label{subsec:dataset_and_models}
% We use the TinySOL dataset which contains 2913 audio clips with a single note played from a single instrument out of a set of 14 instrument classes. This dataset has been chosen as it has consistent recording settings without noise, it is a simple dataset for instrument recognition and finally, confounding factors (compression, sampling rate etc) are minimized.

% We consider 3 models in total:

% \begin{enumerate}
%     \item \textbf{Music/Speech CLAP}:~\cite{clap_learning_audio_concepts_elizalde_2023, laion_clap_Wu_2023} A CLAP-based model trained on music/speech data\footnote{music\_speech\_epoch\_15\_esc\_89.25.pt}
%     \item \textbf{Music CLAP}:~\cite{laion_clap_Wu_2023} A CLAP-based model trained on music data\footnote{music\_audioset\_epoch\_15\_esc\_90.14.pt}
%     \item \textbf{MusCALL}: A version of ~\cite{muscall_manco_2022}, retrained on music data\footnote{https://github.com/ilaria-manco/muscall}
% \end{enumerate}

% We use the two pretrained CLAP systems provided by LAION\footnote{https://github.com/LAION-AI/CLAP}.
% For this work, the original MusCALL implementation was retrained from scratch, as both the data and trained models used in the original paper are not publicly available. 

% We train the MusCALL model from scratch on the LPMusicCaps-MTT~\cite{Doh2023LPMusicCapsLP} dataset, which is built by leveraging the audio and 188 tags from Magna Tag A Tune\cite{Law2009EvaluationOA} to artificially generate captions through a GPT-3.5 model.

% The audio is resampled to 44.1 and 16 KHz for CLAP and MusCALL respectively, and the pre-processing steps described in their respective code repositories are followed.

% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}[b]{\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/muscall_prompt_histogram_of_positive_v_negative_similarities_subplot.png}
%         \caption{Histogram of cosine similarity between TinySOL data and MusCALL prompts in joint audio-text space.}
%         \label{fig:positive_negative_histogram_text}
%     \end{subfigure}
%     \\
%     \begin{subfigure}[b]{\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figs/final_audio_only_positive_negative_joint_space.png}
%         \caption{Histogram of cosine similarity between TinySOL audio data and the mean of optimal intra-class audio embeddings in joint audio-text space.}
%         \label{fig:positive_negative_histogram_audio}
%     \end{subfigure}
%     \caption{Histograms of audio and label embeddings for positive and negative pairs. When using textual prompts, the alignment is problematic, as can be seen from the overlap between positive and negative distributions.}
%     \label{fig:similarity_histograms}
% \end{figure}

% \subsection{Zero-shot transfer for instrument classification}\label{subsec:problem_formulation}
% Given an unseen audio segment $x^{*}$, a text label $l^{*}$ and a two-tower system $f(x)$, we want to model the likelihood $P(l^{*} | x^{*})$ based on the embeddings provided by $f(x)$. In more detail and for the general case, $f \mapsto \mathbb{R}^{F}$ is a function that represents a two-tower system and maps audio or text information to a joint audio-text space, where $F$ is the dimension of the joint space. Also, let $\delta: (\mathbb{R}^{F} \text{ x } \mathbb{R}^{F}) \rightarrow \mathbb{R}$ be a function that measures similarity between joint space embeddings. In this approach, we model the $P(l^{*} | x^{*})$ based on $\delta$, as in:

% \begin{equation}\label{eq:likelihood_approximation}
% P(l^{*} | x^{*}) \propto \delta(f(x^{*}), f(l^{*}))
% \end{equation}

% Multiclass classification attributes the most probable class to each recording and equivalently, the one that has the maximum likelihood. Given our approximation, the output class for each recording is:

% \begin{equation}\label{eq:multiclass_classification}
% c^{*} = \argminB_{c \in C} \delta(f(x^{*}), f(c))
% \end{equation}

% for $c \in C$, where $C = \{c_{1}, c_{2}, \cdots, c_{N}\}$ is the set of classes that we are interested in.

% In our work, the embedding similarity function $\delta$ is the cosine similarity:
% \begin{equation}\label{eq:cosine_similarity}
% \delta(e_{1}, e_{2}) = \frac{e_{1} 
% \cdot e_{2}}{ \lVert e_{1}\rVert \cdot  \lVert e_{2} \rVert}
% \end{equation}

% where $\lVert\cdot\rVert$ is the $L_2$ norm and $e_{i} \in \mathbb{R}^F$ are embeddings.

% \subsection{Are two-tower systems context dependent?}\label{subsec:are_two_tower_systems_context_dependent}
% Two-tower systems are typically not trained on single words, but rather longer prompts. As a result, embedding produced for a single-word text label can result in a very different embedding than a longer prompt. For example, the embedding for the text ``guitar'' may be very different from the embedding for the text ``A guitar track''. When using two-tower models in the context of classification, the class label can be wrapped in a prompt such as ``A <label> track''~\cite{muscall_manco_2022}. As far as we are concerned, we are the first to evaluate the use of more than one type of prompt to test the robustness of two-tower systems during inference. Methods to introduce stochasticity in the prompts used during training have been empirically proven to lead to more robust results~\cite{toward_universal_text_to_music_retrieval_doh_2023}. Retraining the systems and testing different ways of augmenting captions used for training is left for future work, while works in image-text~\cite{8953669} and video-text~\cite{modalit_balanced_embedding_wang_2022} two-tower systems provide some evidence for their usefulness.
% The extent to which text embeddings are currently able to leverage additional textual context is not well understood.

% We explore this effect for each system by slightly changing the text prompt used for zero-shot classification in order to better understand to which extend these systems leverage contextual information. Specifically, we evaluate CLAP models against 6 different prompts:

% \begin{enumerate}
%    \item MusCALL prompt: ``\textit{A <label> track}''
%    \item Generated definition: ``\textit{The <label> is a ...}''
%     \item Definitions without label words: ``\textit{The <removed> is a ...}''
%     \item Label word with random context: ``\textit{<label> <randomly selected lorem ipsum segment>}''
%     \item Musically informed \#1: ``\textit{This is a recording of a <label>}''
%     \item Musically informed \#2: ``\textit{Solo musical instrument sound of a <label>}''
% \end{enumerate}

% The first prompt proposed is a generic prompt that was used in MusCALL. The second prompt is generated using GPT-3.5~\cite{Brown2020LanguageMA}. The third prompt is the same as the second but we removed all instances of the label itself to evaluate the influence of the context on its own. In order to evaluate if the systems are sensitive to specific words and to further evaluate if the context is useful, the fourth prompt adds random words alongside the class text. Lastly, we test 2 musically informed prompts.

% \subsection{Inspecting the cosine similarity distribution}\label{subsec:closely_inspecting_the_cosine_similarity_distribution}
% As a first experiment, we calculate the cosine similarity between the joint space embeddings of each recording from TinySOL and each MusCALL prompt, and compare the similarities of positive pairs vs negative pairs. We define a positive pair as the audio-label pair where the label corresponds to the instrument in the recording, and the negative pairs are all other pairs. Figure~\ref{fig:similarity_histograms}(a) shows histograms of similarities for positive pairs and negative pairs. If the audio-text coherence is good, positive and negative histograms should be well separated.

% To quantify the classification confidence, we calculate the histogram of the difference between the top-2 candidates classes for each recording~\cite{active_learning_survey_aggrawal_2014}. The similarity between each audio embedding and the 14 prompts is estimated and they are sorted in descending order. The difference between top-2 similarities for each song is then calculated and a histogram of that difference is plotted. 

% % Given that the audio embeddings are not entangled and the alignment between text and audio is good, the median value of that difference has to be high, such that the model is confident in its prediction.

% % Lastly and as an auxiliary evaluation of the quality of representations from the audio branch, the mean distance of intra and inter-class audio is calculated, a t-SNE plot is provided and a Logistic Regression model is trained to prove that the audio embeddings are separable and the only issue lies within the text branch

% \begin{figure*}
%  \centerline{\includegraphics[width=0.9\linewidth]{figs/final_prompt_evaluation.png}}
%  \caption{Metrics for 6 textual prompts (See Section~\ref{subsec:are_two_tower_systems_context_dependent}), 2 audio based label embeddings (See section~\ref{subsec:how_far_off_are_we_from_the_optimal_alignment}) and the 3 two-tower multimodal systems. The top row contains top-1 through top-3 accuracy and the bottom Receiver Operating Characteristic and Precision-Recall Area Under the Curve (ROC-AUC and PR-AUC respectively).}
%  \label{fig:prompt_evaluation}
% \end{figure*}

% \subsection{How far-off are we from the ``optimal'' alignment?}
% \label{subsec:how_far_off_are_we_from_the_optimal_alignment}
% To further evaluate if the audio encoder produces meaningful representations, we use the mean of intra-class song embeddings as the label embedding. In detail, we generate the embeddings in the pre-joint and joint audio-text space for each song. Then, we collect the songs that belong to k-th class $c_{k}$ and estimate the mean of the embeddings. The latter serves as the optimal embedding that the text label would have to be mapped to in order to maximize performance. Note that this embedding is only optimal in the case of TinySOL data.
% % Figure~\ref{fig:positive_negative_histogram_audio}

% \subsection{Quantitative evaluation of the text branch}\label{subsec:the_problem_of_evaluating_the_text_branch}
% While there are datasets that can be used to quantify the semantic properties and/or quality of a LM, there isn't one that focuses on music. To overcome this lack of text data for the case of instrument recognition, we can utilise instrument ontologies, which encompass semantic similarity of instruments at multiple levels. We propose to leverage them to quantify the semantic similarity between different instruments and instrument families. In this experiment we use the instrument ontology by Henry Doktorski\footnote{https://free-reed.net/} (HDIO). Note that multiple ontologies have been proposed and each presents limitations~\cite{knowledge_representation_issues_instrument_kolozali_2011}. Repeating the same experiment with other ontologies is left for future work.

% % We extract the tree based on HDIO and calculate cosine similarity between each instrument label in TinySOL. 

% We extract the tree based on HDIO and form every possible triplet of TinySOL instruments label in the tree for a total of 1092 ($91 = {14\choose2}$ combinations of positive word pairs without repetition, multiplied by 12 remaining instruments). The triplets are of the form \emph{(<anchor>, <positive>, <negative>)} where the \emph{<anchor>} label has to be more semantically similar to the \emph{<positive>} than the \emph{<negative>}. Subsequently, every \emph{(<anchor>, <positive>)} pair that is linked through the root node of HDIO is excluded. The number of remaining and valid triplets is 273.

% As a way to quantify semantic meaningfulness with respect to instruments, we calculate cosine similarity between the \emph{(<anchor>, <positive>)} and \emph{(<anchor>, <negative>)} pairs for each system and count the triplets for which the similarity is higher for the first pair than the second.

% We repeat this procedure and form every valid triplet from the ontology, as opposed to just using the instrument labels appearing in TinySOL. As there are $\approx 443k$ triplets, closer examination of the validity and usefulness of specific triplet cases (e.g. ``stringed'', ``plucked'', ``violin'') is left for future work.

% \subsection{Does joint space mapping introduce noise?}
% To further examine the origins of the problematic alignment, we repeat the experiments described in sections \ref{subsec:how_far_off_are_we_from_the_optimal_alignment} and \ref{subsec:the_problem_of_evaluating_the_text_branch} with the embeddings in the audio space and text space before the joint audio-text space mapping.

% \section{Results and discussion}
% Figure \ref{fig:prompt_evaluation} presents the zero-shot instrument recognition results for two CLAP and one MusCALL model with 6 prompts and the audio-only alternatives described in section \ref{subsec:how_far_off_are_we_from_the_optimal_alignment}. Despite additional music data used, Music CLAP performs worse than Music/Speech CLAP for the optimal audio-only zero-shot scenario as well as the top-1 accuracy. 

% The problem with modality alignment can be seen across every model, as metrics almost double when using the audio-only zero-shot scenario which is presented in figure~\ref{fig:positive_negative_histogram_audio}. MusCALL is underfitted and the top-1 accuracy is worse than random for 4 out of 6 textual prompts. This phenomenon might occur due to the small size of training data used, the absence of instrument-specific captions or their underrepresentation in the captions used, as well as the absence of single-note recordings in LPMusicCaps-MTT. While the metrics are low for MusCALL in most of the cases, a large performance increment is still evident for the audio-only scenario which provides more evidence that the problem lies in the audio-text alignment. Also, the audio embeddings seem to be of good quality before and after the projection to the joint audio-text space. This can be seen as the metrics are almost the same before and after projection. 

% Due to very low performance and worse than random results, MusCALL will be excluded from the remaining analysis and training with LP-MSD and re-evaluation is left for future work.

% Apart from that, the performance of CLAP models seems to be heavily correlated with the instrument labels. Removing the label from definitions provide evidence that relevant context cannot be leveraged properly. Also, using musically informed prompts doesn't always result in greater or even comparable results. Specifically, when using the second musically informed prompt for Music CLAP every metric drops considerably.

% CLAP models cannot leverage extra context in the input prompt effectively. Every model performed worse when using relevant context without the instrument word. It seems that the textual encoders put a lot more emphasis on the presence of specific words rather than the meaning of the prompts themselves. In addition, using a generic prompt provided better results than a musically informed one. One counter-example is present with Music CLAP and first musically informed prompt. Furthermore, any kind of context added at the prompts seems to harm the performance in most of the cases and provide more evidence that the model's text encoder cannot properly decompose the sentence to its constituents, use these semantically. Despite this observation, using definitions as prompts seems promising for Music CLAP and every metric apart from top-1 accuracy.

% The relation between sentence and word embeddings is not as straightforward as with bag-of-words LMs~\cite{factors_affecting_sentence_similarity_Alian_2020}. We believe that applying text augmentation for prompts during training (e.g. random masking, word swaps, decomposing a prompt to its parts, or substituting a word with definitions) might be useful for robustness concerning different prompt types, inferring instruments through side information and obtaining good enough embeddings for sentence constituents~\cite{Pratt_2023_ICCV, Ge_2023_CVPR}. Therefore, the utilization of definitions for better inference, as well as their useability during training, is left as future work.

% Positive and negative similarities are very entangled and as a result, retrieval is far from optimal. This is presented in figure \ref{fig:positive_negative_histogram_text}. Fundamentally, a caption is a multi-faceted sentence. We suspect that treating a sentence as only one embedding point (mean of word embeddings) is fundamentally problematic and greatly hinders the semantic properties of the joint space. A hypothesis that needs testing is that by using composite sentences, a model cannot properly infer the relative embeddings of the sentence constituents. 

% We believe that this poses a direct threat to the usefulness of cosine similarity as a way to approximate the conditional likelihood of a label with respect to a song. It is important to underline that even when the metrics reported are good, conclusions about the usefulness of the embeddings cannot be drawn, as equation \ref{eq:multiclass_classification} only utilizes the similarities comparatively. As a result, using two-tower systems off-the-shelf might not be very useful for multi-label scenarios.

% MusCALL seems to be confident in its prediction based on top-2 class similarity differences presented in figure \ref{fig:top_2_confidence_difference}, which is counter intuitive based on the metrics reported. The opposite can be stated for CLAP models, where despite their better performance, the difference have a median value of 0.05-0.08 and instruments cannot be properly disentangled.

% \begin{figure}
%  \centerline{\includegraphics[width=1\linewidth]{figs/final_model_accuracy_by_subset_multibar.png}}
%  \caption{Semantic meaningfulness quantification leveraging Henry Doktorski's instrument ontology. We evaluated the systems over valid triplets obtained through TinySOL labels, as well as every available triplet obtained from the ontology's labels. Accuracies range from 49-59\% which stress that the models do not properly understand musical instruments in depth.}
%  \label{fig:model_accuracy_by_subset}
% \end{figure}

% Apart from evaluating the multimodal alignment for these systems, there is a need to quantify their semantic properties independently~\cite{Roussinov2023} and ways to use captions more effectively, as sentence similarity seems to be senseitive to several factors~\cite{factors_affecting_sentence_similarity_Alian_2020}. As a result, we believe that it is essential for a music terminology similarity corpus to be established. The benefits will be two-fold: (1) it will provide a useful way of quantifying the semantic meaningfulness of the textual branch for two-tower model and (2) it can serve as a baseline to quantify the need for music-informed fine-tuning. The corpus needs to include both musicological terminology as well as informal phrases used to describe music to reduce the potential domain shift between the captions used during training, inference and the sentences that are part of the corpus.

% In this direction, we use HDIO to quantify the semantic quality of the textual branch for 3 systems. Accuracies are presented in figure \ref{fig:model_accuracy_by_subset}. Half of the triplets are not correct and this means that abstract semantic relations between instruments are not effectively captured in the textual branch. We believe that this is an indication of the need for fine-tuning textual encoders on music related data. Despite this fact, it is important to highlight that several instruments and instrumet categories are words that are very frequently used and potentially, almost absent from captions. Experimenting with multiple ontologies and other tasks (e.g. genre recognition) as well as evaluating the importance of the triplets generated is left for future work.

% \section{Conclusion}

% In this paper, we evaluated 3 two-tower multimodal systems for instrument classification. Apart from presenting classification metrics and intra-model comparisons, we provided an elaborate evaluation of the audio and text embeddings in the pre-joint and joint audio-text spaces, and proposed a novel way to quantify the semantic meaningfulness of musical instruments in the textual branch based on triplets derived from an instrument ontology.

% Generally, experiments showed that audio encoders are usually of good quality and as a result, the alignment problem might be traced back to the text branch and/or the joint audio-text space mapping. Two-tower systems appear to lack robustness when it comes to the chosen prompt. Also, they seem to be very senstive to the presence of label words and cannot leverage relevant context.

% Additionally, the audio-label cosine similarities histogram showcased that there is a significant overlap between positive and negative pairs of audio-prompt embedding similarity. This indicates that transcending from multiclass to multilabel classification with two-tower systems is not straightforward, as we cannot use the audio-text cosine similarity directly.

% Finally, more ontologies used to generate triplets need to be tested for instrument recognition, while this methodology can be applied to genre or music emotion ontologies as well.

% \bibliography{ISMIRtemplate}



% % \begin{table*}[!ht]
% %     \begin{center}
% %     \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
% %     \hline
% %         model & prompt & top-1 & top-2 & top-3 & top-4 & top-5 & F1 & ROC-AUC & PR-AUC \\ \hline \hline
% %         audio\_clap & muscall\_prompt & 49.6 & 73.8 & 85.3 & 91.3 & 94.6 & 47.7 & 88.3 & 38.6 \\ \hline
% %         audio\_clap & definition & 33.7 & 55.3 & 69.2 & 77.8 & 86.4 & 29.3 & 89.5 & 39.5 \\ \hline
% %         audio\_clap & definition\_no\_label\_word & 16.9 & 32.9 & 36.7 & 42.9 & 51.9 & 9.8 & 71.8 & 17.9 \\ \hline
% %         audio\_clap & label\_random\_context & 27.1 & 49.3 & 60.2 & 70.6 & 79.8 & 23.1 & 88.4 & 40.1 \\ \hline
% %         audio\_clap & negative\_muscall\_prompts & 31.4 & 47.9 & 64.5 & 75.5 & 80.1 & 28 & 81 & 26.3 \\ \hline
% %         audio\_clap & solo\_musical\_instrument & 43.2 & 63.7 & 73.2 & 79.9 & 86.3 & 42.1 & 89.7 & 38.8 \\ \hline
% %         audio\_clap & this\_is\_a\_recording\_of & 43.4 & 69.6 & 79 & 84.8 & 89.2 & 44.2 & 91.3 & 45.5 \\ \hline
% %         audio\_clap & audio\_only & 89.3 & 98 & 99.3 & 99.7 & 99.8 & 89.3 & 98.1 & 81.1 \\ \hline
% %         audio\_clap & audio\_only\_pre\_projected & 87.7 & 97.3 & 99.4 & 99.7 & 99.9 & 87.7 & 97.3 & 74.6 \\ \hline
% %         music\_clap & muscall\_prompt & 45.3 & 64.4 & 79 & 87.2 & 92.9 & 42.1 & 87.6 & 43.9 \\ \hline
% %         music\_clap & definition & 41.6 & 74.1 & 86.5 & 92.3 & 94.9 & 42.5 & 92 & 50.1 \\ \hline
% %         music\_clap & definition\_no\_label\_word & 18.7 & 32 & 39.8 & 47.6 & 54.1 & 11 & 74.7 & 20.7 \\ \hline
% %         music\_clap & label\_random\_context & 33.8 & 56.7 & 67.7 & 76.9 & 82.2 & 27.6 & 88.2 & 43.9 \\ \hline
% %         music\_clap & negative\_muscall\_prompts & 24.6 & 46.4 & 59.6 & 67.7 & 75.6 & 17.6 & 76.6 & 28.3 \\ \hline
% %         music\_clap & solo\_musical\_instrument & 24.6 & 46.8 & 69.8 & 79.1 & 85.2 & 26.2 & 85.5 & 38.4 \\ \hline
% %         music\_clap & this\_is\_a\_recording\_of & 45.8 & 65.6 & 78.1 & 86.3 & 92 & 42.2 & 93.9 & 55.8 \\ \hline
% %         music\_clap & audio\_only & 86.7 & 97.2 & 99 & 99.5 & 99.6 & 86.7 & 97.3 & 77.4 \\ \hline
% %         music\_clap & audio\_only\_pre\_projected & 84 & 96.2 & 98.6 & 99.1 & 99.7 & 84 & 96.1 & 68.7 \\ \hline
% %         muscall & muscall\_prompt & 4.39 & 14.35 & 23.21 & 35.32 & 44.9 & 1.69 & 56.18 & 8.89 \\ \hline
% %         muscall & definition & 4.6 & 8.41 & 12.7 & 21.97 & 26.64 & 1.53 & 53.97 & 8.66 \\ \hline
% %         muscall & definition\_no\_label\_word & 3.54 & 6.87 & 10.23 & 16.48 & 23.65 & 0.32 & 53.93 & 8.94 \\ \hline
% %         muscall & label\_random\_context & 11.05 & 30.79 & 40.89 & 44.73 & 48.27 & 4.58 & 60.11 & 11.03 \\ \hline
% %         muscall & negative\_muscall\_prompts & 3.84 & 13.97 & 24.1 & 42.29 & 50.57 & 1.19 & 54.92 & 8.46 \\ \hline
% %         muscall & solo\_musical\_instrument\_sound\_of & 10.54 & 16.58 & 22.31 & 28.18 & 35.98 & 4.55 & 55.52 & 8.58 \\ \hline
% %         muscall & this\_is\_a\_recording\_of & 6.39 & 16.62 & 38.21 & 43.29 & 46.93 & 3.17 & 56.21 & 8.95 \\ \hline
% %         muscall & audio\_only & 47.6 & 65.6 & 73.6 & 79.3 & 85.2 & 47.9 & 71.6 & 27.6 \\ \hline
% %         muscall & audio\_only\_pre\_projected & 48.4 & 65.2 & 73.3 & 79.5 & 85 & 48.3 & 72.1 & 27.9 \\ \hline
% %     \end{tabular}
% %     \end{center}
% %      \caption{Ablation study with two CLAP models trained in audio and music data respectively. Those systems are zero-shot evaluated using different prompts.}
% %      \label{tab:ablation_zero_shot_evaluation}
% % \end{table*}


% \end{document}


